Recurrent Neural Networks for anomaly detection in the Post-Mortem time series of LHC superconducting magnets

This paper presents a model based on Deep Learning algorithms of LSTM and GRU for facilitating an anomaly detection in Large Hadron Collider superconducting magnets. We used high resolution data available in Post Mortem database to train a set of models and chose the best possible set of their hyper-parameters. Using Deep Learning approach allowed to examine a vast body of data and extract the fragments which require further experts examination and are regarded as anomalies. The presented method does not require tedious manual threshold setting and operator attention at the stage of the system setup. Instead, the automatic approach is proposed, which achieves according to our experiments accuracy of 99%. This is reached for the largest dataset of 302 MB and the following architecture of the network: single layer LSTM, 128 cells, 20 epochs of training, look_back=16, look_ahead=128, grid=100 and optimizer Adam. All the experiments were run on GPU Nvidia Tesla K80

==> ack.tex <==
\section*{Acknowledgment}
I would like to thank my wife Urszula Wielgosz for her huge contribution to the preparation of the paper.

==> contents-10-system-description.tex <==
\section{System description}
\label{section:system_description}

The LHC as an experimental device is composed of many components which constitute a large system. The tunnel and the accelerator is just a very critical tiny fraction of the LHC infrastructure. 
This research revolves around three main components of the machine, namely superconducting magnets \cite{LHCDesRep}, Quench Protection System \cite{qps, qps_fpga} and the Post-mortem database. 
The two first elements were comprehensively presented in \cite{wielgosz2016usingLSTM} and thus will not be address in this paper.

This section is mostly focus on introduction to the CERN Post-Mortem database in a context of the research and the experiments conducted as a part of this work. 


